MM-UAVBench: How Well Do Multimodal Large Language Models See, Think, and Plan in Low-Altitude UAV Scenarios?

While Multimodal Large Language Models (MLLMs) have exhibited remarkable general intelligence across diverse domains, their potential in low-altitude applications dominated by Unmanned Aerial Vehicles (UAVs) remains largely underexplored. Existing MLLM benchmarks rarely cover the unique challenges of low-altitude scenarios, while UAV-related evaluations mainly focus on specific tasks such as localization or navigation, without a unified evaluation of MLLMs'general intelligence. To bridge this gap, we present MM-UAVBench, a comprehensive benchmark that systematically evaluates MLLMs across three core capability dimensions-perception, cognition, and planning-in low-altitude UAV scenarios. MM-UAVBench comprises 19 sub-tasks with over 5.7K manually annotated questions, all derived from real-world UAV data collected from public datasets. Extensive experiments on 16 open-source and proprietary MLLMs reveal that current models struggle to adapt to the complex visual and cognitive demands of low-altitude scenarios. Our analyses further uncover critical bottlenecks such as spatial bias and multi-view understanding that hinder the effective deployment of MLLMs in UAV scenarios. We hope MM-UAVBench will foster future research on robust and reliable MLLMs for real-world UAV intelligence.

==> main_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/blind_evaluation.tex <==
\begingroup
% \definecolor{perceptionColor}{HTML}{87CEEB} 
\definecolor{perceptionColor}{HTML}{96A9BF} 
% \definecolor{cognitionColor}{HTML}{DDA0DD}   
\definecolor{cognitionColor}{HTML}{EBD8B7}
% \definecolor{planningColor}{HTML}{FFA07A}   
\definecolor{planningColor}{HTML}{B5A69C}   
% \definecolor{oai-gray-600}{RGB}{130, 130, 130}
% \definecolor{oai-gray-600}{RGB}{108, 100, 158}
\definecolor{oai-gray-600}{RGB}{232, 159, 44}
% \definecolor{oai-gray-300}{RGB}{220, 220, 220}  
% \definecolor{oai-gray-300}{RGB}{173, 168, 208} 
\definecolor{oai-gray-300}{RGB}{254, 210, 103}
\definecolor{oai-red-1}{RGB}{250, 40, 55}
\definecolor{oai-red-2}{RGB}{255, 110, 120}
\definecolor{oai-red-3}{RGB}{247, 198, 198}

% 导言区需提前加载：\usepackage{graphicx}、\usepackage{xcolor}
\begin{table*}[ht!]  % 自动占满双栏宽度
    \captionsetup{type=table}
    \caption{\textbf{Blind evaluation results on \textbf{\OURS}.}}
    \vspace{-0.3em}
    \centering
    \fontsize{6pt}{7pt}\selectfont  % 增大字体提升可读性
    \setlength\tabcolsep{3pt}  % 拉宽列间距（原2pt→4pt，可按需微调）
    \renewcommand{\arraystretch}{1.5}  % 增大行高，避免文字拥挤
    \begin{tabular}{r|c|cccccccccccccccccccc}
       & &
        \rotatebox{75}{Scene. Class.} &
        \rotatebox{75}{Orient. Class.} &
        \rotatebox{75}{Env. State} & 
        \rotatebox{75}{Urban OCR} &
        \rotatebox{75}{CA. Count} &
        \rotatebox{75}{RE. Count} &
        \rotatebox{75}{Target Back.} &
        \rotatebox{75}{Cross-Obj R.} &
        \rotatebox{75}{Intent Anal.} &
        \rotatebox{75}{Scene Attri.} &
        \rotatebox{75}{Scene Damage} &
        \rotatebox{75}{Scene Pred.} &
        \rotatebox{75}{Event Trace} &
        \rotatebox{75}{Event Under.} &
        \rotatebox{75}{Event Pred.} &
        \rotatebox{75}{Temporal Order} &
        \rotatebox{75}{Swarm Plan} &
        \rotatebox{75}{Ground Plan} &
        \rotatebox{75}{Air-Ground Plan} \\
        Methods & Avg. & 
        \multicolumn{6}{c}{\cellcolor{perceptionColor!50}Perception} & 
        \multicolumn{10}{c}{\cellcolor{cognitionColor!50}Cognition} & 
        \multicolumn{3}{c}{\cellcolor{planningColor!50}Planning} \\
        \hline
        
        Qwen3-VL-8B &  \\
        Qwen3-VL-32B &  \\
        Qwen2.5-VL-7B & \\
        Qwen2.5-VL-32B &  \\
        Qwen2.5-VL-72B &  \\
        InternVL3.5-8B &  \\
        InternVL3.5-38B &  \\
        InternVL3-14B &  \\
        InternVL3-78B&  \\
        LLaVA-OneVision-7B &  \\

        \hline
    \end{tabular}
    \label{tab:zero_shot_all}
\end{table*}
\endgroup

==> tables/quality_control.tex <==
\begingroup
\renewcommand{\arraystretch}{1.8}  % 增大行高，提升可读性
\setlength\tabcolsep{5pt}  % 列间距微调（原6pt→5pt，进一步压缩列间空白）
\begin{table*}[ht!]
    \centering
    \fontsize{9pt}{11pt}\selectfont
    \caption{Quality Control Measures for Annotation Refinement}
    \label{tab:annotation_quality_control}
    % 第一列宽3cm，第二列宽2.5cm，后两列按比例调整（总宽度适配双栏）
    \begin{tabular}{p{3cm}|p{2.5cm}|p{5.5cm}|p{6.5cm}}
        \toprule
        \textbf{Quality Control} & \textbf{Issue} & \textbf{Refinement} & \textbf{Examples} \\
        \midrule
        \multirow{3}{=}{Annotation Accuracy Control} 
        & Viewpoint Ambiguity 
        & Explicit Reference Frame Definition 
        & from the camera’s perspective… \\
        \cmidrule(lr){2-4}
        & Ambiguous Lane Descriptions 
        & Template: \newline
          ``vehicles in the [lane] of the [direction] [approach]'' \newline
          $\bullet$ Approach: Horizontal / Vertical \newline
          $\bullet$ Direction: \newline
            \quad - Horizontal: Left-to-Right / Right-to-Left \newline
            \quad - Vertical: Bottom-to-Top / Top-to-Bottom \newline
          $\bullet$ Lane: Inner / Middle / Outer / Non-motorized
        & ``...vehicles in the inner lane of the left-to-right horizontal approach'' \\
        \cmidrule(lr){2-4}
        & Ambiguous Optimization Objectives 
        & Explicit Prioritization Constraints \newline
          Priority Rule: Severity of Damage $\gg$ Flight Distance \newline
          and add restriction to question
        & $\bullet$ Original (Ambiguous): ``...plan the most reasonable route that is fast and efficient and shortens the rescue time...'' \newline
          $\bullet$ Refined (Explicit): ``...plan the most reasonable route that prioritizes damage severity while shortening the rescue time...'' \\
        \bottomrule
    \end{tabular}
\end{table*}
\endgroup

==> tables/spatial_bias_detailed.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\sisetup{
  table-format=1.3,
  detect-weight=true,
  detect-inline-weight=math,
  input-decimal-markers=.,
}
\begin{tabular}{l|l||*{4}{S}}
\toprule
\textbf{Model} & \textbf{Answer} & \textbf{Straight} & \textbf{Right} & \textbf{Left} & \textbf{Stationary} \\
\midrule
GPT-4o & Straight   & 0.347 & 0.149 & 0.079 & 0.426 \\
       & Right      & 0.363 & 0.176 & 0.118 & 0.343 \\
       & Left       & 0.294 & 0.147 & 0.206 & 0.353 \\
       & Stationary & 0.353 & 0.108 & 0.029 & 0.510 \\
\midrule
Qwen2.5-VL-72B-Instruct & Straight   & 0.490 & 0.000 & 0.000 & 0.500 \\
                        & Right      & 0.431 & 0.000 & 0.000 & 0.569 \\
                        & Left       & 0.490 & 0.020 & 0.000 & 0.490 \\
                        & Stationary & 0.402 & 0.000 & 0.000 & 0.598 \\
\midrule
InternVL3-78B & Straight   & 0.696 & 0.059 & 0.069 & 0.176 \\
              & Right      & 0.490 & 0.098 & 0.265 & 0.147 \\
              & Left       & 0.627 & 0.049 & 0.206 & 0.118 \\
              & Stationary & 0.480 & 0.098 & 0.098 & 0.324 \\
\midrule
Qwen2.5-VL-32B-Instruct & Straight   & 0.284 & 0.284 & 0.363 & 0.069 \\
                        & Right      & 0.186 & 0.147 & 0.569 & 0.098 \\
                        & Left       & 0.314 & 0.225 & 0.382 & 0.078 \\
                        & Stationary & 0.186 & 0.176 & 0.529 & 0.108 \\
\midrule
InternVL3-14B & Straight   & 0.294 & 0.392 & 0.284 & 0.029 \\
              & Right      & 0.167 & 0.343 & 0.471 & 0.020 \\
              & Left       & 0.255 & 0.343 & 0.392 & 0.010 \\
              & Stationary & 0.245 & 0.471 & 0.216 & 0.069 \\
\midrule
InternVL3-8B & Straight   & 0.255 & 0.500 & 0.245 & 0.000 \\
             & Right      & 0.167 & 0.520 & 0.304 & 0.010 \\
             & Left       & 0.343 & 0.402 & 0.255 & 0.000 \\
             & Stationary & 0.333 & 0.520 & 0.147 & 0.000 \\
\midrule
MiniCPM-V-4.5 & Straight   & 0.480 & 0.225 & 0.275 & 0.020 \\
              & Right      & 0.373 & 0.392 & 0.235 & 0.000 \\
              & Left       & 0.382 & 0.235 & 0.353 & 0.029 \\
              & Stationary & 0.402 & 0.265 & 0.304 & 0.029 \\
\midrule
Qwen2.5-VL-7B-Instruct & Straight   & 0.412 & 0.127 & 0.402 & 0.059 \\
                       & Right      & 0.275 & 0.324 & 0.402 & 0.000 \\
                       & Left       & 0.451 & 0.088 & 0.431 & 0.029 \\
                       & Stationary & 0.441 & 0.118 & 0.431 & 0.010 \\
\bottomrule
\end{tabular}
\caption{Model Prediction Bias}
\label{tab:spatial_bias}
\end{table*}



==> tables/spatial_bias_overall.tex <==
\begin{table}[t]
\centering
\caption{Prediction Accuracy (\%)}
\label{tab:prediction_accuracy}
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\sisetup{
  table-format=1.4,        % 对齐至小数点，最多1位整数+4位小数
  detect-weight=true,
  detect-inline-weight=math,
  input-decimal-markers=.,
}
\begin{tabular}{l| *{5}{S}}
\toprule
\textbf{Model} & \textbf{Straight} & \textbf{Right} & \textbf{Left} & \textbf{Stationary} & \textbf{Average} \\
\midrule
GPT-4o & 0.3431 & 0.1765 & 0.2059 & 0.5098 & 0.5098 \\
Qwen2.5-VL-72B-In & 0.4902 & 0 & 0 & 0.598 & 0.598 \\
InternVL3-78B & 0.6961 & 0.098 & 0.2059 & 0.3235 & 0.3235 \\
Qwen2.5-VL-32B-In & 0.2843 & 0.1471 & 0.3824 & 0.1078 & 0.1078 \\
InternVL3-14B & 0.2941 & 0.3431 & 0.3922 & 0.0686 & 0.0686 \\
InternVL3-8B & 0.2549 & 0.5196 & 0.2549 & 0 & 0 \\
MiniCPM-V-4.5 & 0.4804 & 0.3922 & 0.3529 & 0.0294 & 0.0294 \\
Qwen2.5-VL-7B-In & 0.4118 & 0.3235 & 0.4314 & 0.0098 & 0.0098 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/spatial_bias_revise.tex <==
\begin{table*}[t]
\centering
\small
% ===== InternVL 系列 =====
\begin{subtable}[t]{0.32\textwidth}
\centering
\caption{InternVL3-78B}
\begin{tabular}{l|cccc}
\toprule
 & Str & Ri & Le & St \\
\midrule
Str & .696 & .059 & .069 & .176 \\
Ri  & .490 & .098 & .265 & .147 \\
Le  & .627 & .049 & .206 & .118 \\
St  & .480 & .098 & .098 & .324 \\
\bottomrule
\end{tabular}
\end{subtable}
\hfill
\begin{subtable}[t]{0.32\textwidth}
\centering
\caption{InternVL3-14B}
\begin{tabular}{l|cccc}
\toprule
 & Str & Ri & Le & St \\
\midrule
Str & .294 & .392 & .284 & .029 \\
Ri  & .167 & .343 & .471 & .020 \\
Le  & .255 & .343 & .392 & .010 \\
St  & .245 & .471 & .216 & .069 \\
\bottomrule
\end{tabular}
\end{subtable}
\hfill
\begin{subtable}[t]{0.32\textwidth}
\centering
\caption{InternVL3-8B}
\begin{tabular}{l|cccc}
\toprule
 & Str & Ri & Le & St \\
\midrule
Str & .255 & .500 & .245 & .000 \\
Ri  & .167 & .520 & .304 & .010 \\
Le  & .343 & .402 & .255 & .000 \\
St  & .333 & .520 & .147 & .000 \\
\bottomrule
\end{tabular}
\end{subtable}

\vspace{3mm}
% ===== QwenVL 系列 =====
\begin{subtable}[t]{0.32\textwidth}
\centering
\caption{Qwen2.5-VL-72B-Instruct}
\begin{tabular}{l|cccc}
\toprule
 & Str & Ri & Le & St \\
\midrule
Str & .490 & .000 & .000 & .500 \\
Ri  & .431 & .000 & .000 & .569 \\
Le  & .490 & .020 & .000 & .490 \\
St  & .402 & .000 & .000 & .598 \\
\bottomrule
\end{tabular}
\end{subtable}
\hfill
\begin{subtable}[t]{0.32\textwidth}
\centering
\caption{Qwen2.5-VL-32B-Instruct}
\begin{tabular}{l|cccc}
\toprule
 & Str & Ri & Le & St \\
\midrule
Str & .284 & .284 & .363 & .069 \\
Ri  & .186 & .147 & .569 & .098 \\
Le  & .314 & .225 & .382 & .078 \\
St  & .186 & .176 & .529 & .108 \\
\bottomrule
\end{tabular}
\end{subtable}
\hfill
\begin{subtable}[t]{0.32\textwidth}
\centering
\caption{Qwen2.5-VL-7B-Instruct}
\begin{tabular}{l|cccc}
\toprule
 & Str & Ri & Le & St \\
\midrule
Str & .412 & .127 & .402 & .059 \\
Ri  & .275 & .324 & .402 & .000 \\
Le  & .451 & .088 & .431 & .029 \\
St  & .441 & .118 & .431 & .010 \\
\bottomrule
\end{tabular}
\end{subtable}

\vspace{3mm}
% ===== GPT4o / MiniCPM 系列 =====
\begin{subtable}[t]{0.32\textwidth}
\centering
\caption{GPT-4o}
\begin{tabular}{l|cccc}
\toprule
 & Str & Ri & Le & St \\
\midrule
Str & .347 & .149 & .079 & .426 \\
Ri  & .363 & .176 & .118 & .343 \\
Le  & .294 & .147 & .206 & .353 \\
St  & .353 & .108 & .029 & .510 \\
\bottomrule
\end{tabular}
\end{subtable}
\hfill
\begin{subtable}[t]{0.32\textwidth}
\centering
\caption{MiniCPM-V-4.5}
\begin{tabular}{l|cccc}
\toprule
 & Str & Ri & Le & St \\
\midrule
Str & .480 & .225 & .275 & .020 \\
Ri  & .373 & .392 & .235 & .000 \\
Le  & .382 & .235 & .353 & .029 \\
St  & .402 & .265 & .304 & .029 \\
\bottomrule
\end{tabular}
\end{subtable}
\hfill
\begin{subtable}[t]{0.32\textwidth}
\centering
\caption{GT}
\begin{tabular}{l|cccc}
\toprule
 & Str & Ri & Le & St \\
\midrule
Str & 1. & .0 & .0 & .0 \\
Ri  & .0 & 1. & .0 & .0 \\
Le  & .0 & .0 & 1. & .0 \\
St  & .0 & .0 & .0 & 1. \\
\bottomrule
\end{tabular}
\end{subtable}

\caption{Fuzzy confusion matrices for all evaluated models.  
Each cell denotes the probability of predicting the column action given the ground-truth row action.  
Rows correspond to ground-truth directions (Straight, Right, Left, Stationary).}
\label{tab:fuzzy_confusion}
\end{table*}


==> tables/target_size.tex <==
\captionsetup[table]{font=small}

\sisetup{
  round-mode = places,
  round-precision = 2,
  table-number-alignment = center,
  detect-weight = true,
  input-decimal-markers = {.},
}

\begin{table}[t]
\centering
\caption{
Model performance across target areas (S: bottom 1/3, M: middle 1/3, L: top 1/3 by scale).
Larger targets tend to yield higher accuracy, while small targets remain challenging.
}
\scriptsize
\setlength{\tabcolsep}{5.5pt}
\renewcommand{\arraystretch}{1.5}

\begin{tabular}{l *{3}{S} *{3}{S}}
\toprule
\rowcolor{gray!15}  % 表头行设置浅灰色背景（灰度15%，不刺眼）
\textbf{Model} &
\multicolumn{3}{c}{\textbf{Orientation Classification}} & 
\multicolumn{3}{c}{\textbf{Target Backtracking}} \\
\cmidrule(lr){2-4}\cmidrule(l){5-7}
& {S} & {M} & {L}
& {S} & {M} & {L} \\
\midrule
Qwen2.5-VL-7B    & 28.40 & 29.51 & 35.32 & 47.37 & 51.28 & 51.22 \\
Qwen2.5-VL-72B   & 37.86 & 35.66 & 30.95 & 28.95 & 48.72 & 36.59 \\
Qwen3-VL-8B      & 24.28 & 27.87 & 27.38 & 44.74 & 46.15 & 58.54 \\
Qwen3-VL-32B     & 37.86 & 43.85 & 44.84 & 42.11 & 41.03 & 43.90 \\
InternVL3\_5-8B  & 24.69 & 24.59 & 31.75 & 23.68 & 41.03 & 39.02 \\
InternVL3-78B    & 38.27 & 35.66 & 30.56 & 50.00 & 46.15 & 53.66 \\
\bottomrule
\end{tabular}
\label{tab:target_scale}
\end{table}

==> tables/zero_shot_evaluation.tex <==
\begin{table*}[h]
\centering 
\caption{Performance comparison with other methods on \OURS.} 
\scalebox{0.75}{ 
\begin{tabular}{|c|ccccccc|c|} 
\hline 
\multirow{2}{*}{Models} & \multicolumn{7}{c|}{Perception} & \multirow{2}{*}{Avg.} \\  
\cline{2-8} 
& Scene Class. & Ori. Class. & Environ. State Class. & Visual Loc. & Urban OCR & Obj. Count & Crowd Count & \\  
\hline 
\multicolumn{9}{|l|}{API-based Multimodal LLMs} \\ 
\hline 
GPT-4o & 0.695 & 0.342 & - & - & 0.703 & - & - & -\\ 
\hline  
\multicolumn{9}{|l|}{Open-source Multimodal LMMs} \\ 
\hline 
Qwen2.5-VL-72B-Instruct & 0.711 & 0.326 & - & - & 0.753 & - & - & - \\ 
InternVL3-78B & \textbf{0.736} & \textbf{0.434} & - & - & 0.753 & - & - & - \\ 
Qwen2.5-VL-32B-Instruct & 0.690 & 0.263 & - & - & \textbf{0.775} & -  & - & - \\ 
InternVL3-14B & 0.665 & 0.242 & - & - & 0.725 & - & - & - \\ 
InternVL3-8B & 0.636 & 0.242 & - & - & 0.684 & - & - & - \\ 
MiniCPM-V-4.5 & 0.632 & 0.364 & - & - & 0.741 & - & - & - \\ 
Qwen2.5-VL-7B-Instruct & 0.690 & 0.346 & - & - & 0.706 & - & - & - \\ 
\hline  
\multicolumn{9}{|l|}{Remote Sensing VLMs} \\ 
\hline 
Geochat & - & - & - & - & - & - & - & - \\ 
\hline 
Or\end{tabular} } 
\label{tab:main} 
\end{table*}

\begin{table*}[h]
\centering 
\caption{Performance comparison with other methods on \OURS.} 
\scalebox{0.55}{ 
\begin{tabular}{|c|cccccccccc|c|} 
\hline 
\multirow{2}{*}{Models} & \multicolumn{10}{c|}{Cognition} & \multirow{2}{*}{Avg.} \\  
\cline{2-11} 
& \makecell{Target \\Backtracking} 
& \makecell{Cross-Object \\Reasoning} 
& \makecell{Intent Analysis \\and Prediction} 
& \makecell{Scene Function \\and Attribute Recognition} 
& \makecell{Scene Anomaly \\Detection} 
& \makecell{Scene Analysis \\and Prediction} 
& \makecell{Event \\Tracing} 
& \makecell{Event \\Understanding} 
& \makecell{Event \\Prediction} 
& \makecell{Multi-Image \\Sorting} & \\
\hline 
\multicolumn{12}{|l|}{API-based Multimodal LLMs} \\ 
\hline 


GPT-4o & 0.280 & 0.465 & 0.517 & 0.881 & - & \textbf{0.810} & \textbf{0.738} & 0.763 & 0.563 & 0.272 & -\\ 
Gemini-Pro & - & - & - & - & - & - & - & - & - & - & -\\
\hline  
\multicolumn{12}{|l|}{Open-source Multimodal LMMs} \\ 
\hline 
Qwen2.5-VL-72B-Instruct  & 0.475 & 0.512 & 0.586 & \textbf{0.895} & - & 0.762 & 0.714 & 0.737 & 0.563 & 0.316 & - \\ 
InternVL3-78B  & \textbf{0.534 }& 0.512 & 0.517 & \textbf{0.895} & - & 0.667 & - & - & - & \textbf{0.360} & - \\ 
Qwen2.5-VL-32B-Instruct  & 0.424 & 0.465 & 0.724 & 0.881 & - & \textbf{0.810} & 0.679 & 0.686 & 0.438 & 0.281 & - \\  
InternVL3-14B  & 0.492 & 0.512 & 0.517 & 0.852 & - & 0.476 & \textbf{0.738} & 0.731 & 0.438 & 0.351 & - \\ 
InternVL3-8B  & 0.517 & \textbf{0.576} & 0.621 & 0.874 & - & 0.524 & 0.655 & 0.776 & \textbf{0.688} & 0.351 & - \\ 
MiniCPM-V-4.5  & 0.398 & 0.483 & 0.655 & 0.574 & - & 0.571 & 0.667 & \textbf{0.788} & 0.500 & 0.281 & - \\ 
Qwen2.5-VL-7B-Instruct  & 0.432 & 0.477 & \textbf{0.759} & 0.888 & - & 0.667 & 0.595 & 0.686 & 0.438 & 0.272 & - \\ 
\hline  
\multicolumn{12}{|l|}{Remote Sensing VLMs} \\ 
\hline 
Geochat & - & - & - & - & - & - & - & - & - & - & -\\ 
\hline 
\end{tabular} } 
\label{tab:main} 
\end{table*}

\begin{table*}[h]
\centering 
\caption{Performance comparison with other methods on \OURS.} 
\scalebox{0.8}{ 
\begin{tabular}{|c|cccc|c|} 
\hline 
\multirow{2}{*}{Models} & \multicolumn{4}{c|}{Planning} & \multirow{2}{*}{Avg.} \\  
\cline{2-5} 
& \makecell{ Autonomous Motion \\ Planning} 
& \makecell{Swarm Collaborative \\ Planning}
& \makecell{Semantic-Guided \\ Planning} 
& \makecell{ Situational-Responsive \\ Collaborative Planning} & \\ 
\hline 
\multicolumn{6}{|l|}{API-based Multimodal LLMs} \\ 
\hline 
GPT4o & - & 0.347 & 0.496 & 0.698 & - \\ 
Gemini-Pro & - & - & - & - & - \\
\hline  
\multicolumn{6}{|l|}{Open-source Multimodal LMMs} \\ 
\hline 
Qwen2.5-VL-72B-Instruct & - & 0.389 & \textbf{0.537} & \textbf{0.849} & -  \\ 
InternVL3-78B & - & \textbf{0.458} & 0.507 & 0.736 & -  \\ 
Qwen2.5-VL-32B-Instruct & - & 0.278 & 0.496 & 0.755 & -   \\ 
InternVL3-14B & - & 0.278 & 0.474 & 0.774 & -   \\ 
InternVL3-8B & - & 0.403 & 0.377 & 0.717 & -   \\ 
MiniCPM-V-4.5 & - & 0.431 & 0.448 & 0.755 & -   \\ 
Qwen2.5-VL-7B-Instruct & - & 0.403 & 0.485 & 0.736 & -  \\
\hline  
\multicolumn{6}{|l|}{Remote Sensing VLMs} \\ 
\hline 
Geochat & - & - & - & - & -  \\ 
\hline 
\end{tabular} } 
\label{tab:main} 
\end{table*}


==> tables/zero_shot_evaluation_merged.tex <==
\begin{table*}[t]
\centering
% ========== 局部作用域：siunitx 设置仅对本表生效 ==========
\begingroup
\scriptsize
\fontsize{4}{8.5}\selectfont
\setlength{\tabcolsep}{0.8pt}
\renewcommand{\arraystretch}{0.8}

\sisetup{                     % ← 仅本表有效，不影响其它表
  mode = math,
  tight-spacing = true,
  detect-weight = true,
  detect-family = true,
  round-mode = places,
  round-precision = 2,
  output-decimal-marker = .,
  group-minimum-digits = 4
}

% 均值
\def\avgA{0.543}\def\avgB{0.625}\def\avgC{0.598}\def\avgD{0.587}%
\def\avgE{0.534}\def\avgF{0.551}\def\avgG{0.549}\def\avgH{0.562}

\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{@{} L{1.8cm} | N | *{20}{N} @{}} 
\toprule

% 表头（关键：用固定高的 parbox 保证与旋转列等高且垂直居中）
\parbox[c][\HdrH][c]{1.8cm}{\centering\textbf{Models}} &
\parbox[c][\HdrH][c]{\NumW}{\centering\textbf{Avg.}}
& \rot{Scene. Class.} & \rot{Orient. Class} & \rot{Env. State} & \rot{Urban OCR} & \rot{CA Count} & \rot{REC Count}
& \rot{Target Back.} & \rot{Cross-Obj R.} & \rot{Intent Anal.} & \rot{Scene Func.} & \rot{Scene Damage} & \rot{Scene Anom.}  & \rot{Event Trace} & \rot{Event Under.} & \rot{Event Pred.} & \rot{Multi-Pic. Sort}
& \rot{Swarm Plan} & \rot{Semantic Plan} & \rot{Situational Plan} \\
\midrule

Random & \cellcolorapply{\avgA} & \cellcolorapply{0.695} & \cellcolorapply{0.342} & \cellcolorapply{0.741} & \cellcolorapply{0.500} & \cellcolorapply{0.703} & \cellcolorapply{0.500} & \cellcolorapply{0.500} & \cellcolorapply{0.280} & \cellcolorapply{0.465} & \cellcolorapply{0.517} & \cellcolorapply{0.881} & \cellcolorapply{0.500} & \cellcolorapply{0.810} & \cellcolorapply{0.500} & \cellcolorapply{0.500} & \cellcolorapply{0.500} & \cellcolorapply{0.272} & \cellcolorapply{0.314} & \cellcolorapply{0.467} & \cellcolorapply{0.829} \\

Human & \cellcolorapply{\avgA} & \cellcolorapply{0.695} & \cellcolorapply{0.342} & \cellcolorapply{0.741} & \cellcolorapply{0.500} & \cellcolorapply{0.703} & \cellcolorapply{0.500} & \cellcolorapply{0.500} & \cellcolorapply{0.280} & \cellcolorapply{0.465} & \cellcolorapply{0.517} & \cellcolorapply{0.881} & \cellcolorapply{0.500} & \cellcolorapply{0.810} & \cellcolorapply{0.500} & \cellcolorapply{0.500} & \cellcolorapply{0.500} & \cellcolorapply{0.272} & \cellcolorapply{0.314} & \cellcolorapply{0.467} & \cellcolorapply{0.829} \\
\midrule
% 分组标题：水平居中
\multicolumn{22}{c}{\textit{API-based}} \\
\midrule
GeminiPro-2.5 & \cellcolorapply{\avgA} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.7325} & \cellcolorapply{0.7309} & \cellcolorapply{0.6802} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} \\

GeminiFlash-2.5 & \cellcolorapply{\avgA} & \cellcolorapply{0.7071} & \cellcolorapply{0.4100} & \cellcolorapply{0.6830} & \cellcolorapply{0.7594} & \cellcolorapply{0.2455} & \cellcolorapply{0.3286} & \cellcolorapply{0.3898} & \cellcolorapply{0.5291} & \cellcolorapply{0.2097} & \cellcolorapply{0.8339} & \cellcolorapply{0.4686} & \cellcolorapply{0.4155} & \cellcolorapply{0.7078} & \cellcolorapply{0.6944} & \cellcolorapply{0.6640} & \cellcolorapply{0.2114} & \cellcolorapply{0.1554} & \cellcolorapply{0.3994} & \cellcolorapply{0.2019} \\

GPT-4o(old) & \cellcolorapply{\avgA} & \cellcolorapply{0.695} & \cellcolorapply{0.342} & \cellcolorapply{0.741} & \cellcolorapply{0.000} & \cellcolorapply{0.703} & \cellcolorapply{0.000} & \cellcolorapply{0.000} & \cellcolorapply{0.280} & \cellcolorapply{0.465} & \cellcolorapply{0.517} & \cellcolorapply{0.881} & \cellcolorapply{0.000} & \cellcolorapply{0.810} & \cellcolorapply{0.000} & \cellcolorapply{0.000} & \cellcolorapply{0.000} & \cellcolorapply{0.272} & \cellcolorapply{0.314} & \cellcolorapply{0.467} & \cellcolorapply{0.829} \\

GPT-4o(new) & \cellcolorapply{\avgA} & \cellcolorapply{0.5732} & \cellcolorapply{0.3843} & \cellcolorapply{0.6801} & \cellcolorapply{0.6219} & \cellcolorapply{0.2212} & \cellcolorapply{0.1886} & \cellcolorapply{0.1441} & \cellcolorapply{0.2558} & \cellcolorapply{0.5000} & \cellcolorapply{0.8339} & \cellcolorapply{0.3171} & \cellcolorapply{0.4010} & \cellcolorapply{0.6708} & \cellcolorapply{0.6478} & \cellcolorapply{0.6316} & \cellcolorapply{0.3371} & \cellcolorapply{0.2838} & \cellcolorapply{0.3909} & \cellcolorapply{0.4519} \\

Qwen3-VL-235B-A22B(new) & \cellcolorapply{\avgA} & \cellcolorapply{0.6904} & \cellcolorapply{0.4114} & \cellcolorapply{0.7579} & \cellcolorapply{0.7344} & \cellcolorapply{0.4727} & \cellcolorapply{0.2600} & \cellcolorapply{0.4322} & \cellcolorapply{0.5174} & \cellcolorapply{0.5194} & \cellcolorapply{0.8628} & \cellcolorapply{0.3943} & \cellcolorapply{0.5845} & \cellcolorapply{0.6996} & \cellcolorapply{0.7243} & \cellcolorapply{0.6842} & \cellcolorapply{0.4057} & \cellcolorapply{0.3345} & \cellcolorapply{0.4674} & \cellcolorapply{0.5096} \\

\midrule

\multicolumn{22}{c}{\textit{Open-source}} \\
\midrule
Qwen3-VL-8B   & \cellcolorapply{\avgH} & \cellcolorapply{0.6987} & \cellcolorapply{0.2652} & \cellcolorapply{0.7176} & \cellcolorapply{0.7969} & \cellcolorapply{0.3879} & \cellcolorapply{0.1857} & \cellcolorapply{0.5000} & \cellcolorapply{0.5756} & \cellcolorapply{0.5818} & \cellcolorapply{0.8556} & \cellcolorapply{0.3400} & \cellcolorapply{0.5314} & \cellcolorapply{0.5844} & \cellcolorapply{0.6246} & \cellcolorapply{0.6154} & \cellcolorapply{0.3000} & \cellcolorapply{0.2712} & \cellcolorapply{0.4561} & \cellcolorapply{0.3990} \\

Qwen3-VL-32B  & \cellcolorapply{\avgD} & \cellcolorapply{0.6862} & \cellcolorapply{0.4181} & \cellcolorapply{0.7522} & \cellcolorapply{0.7656} & \cellcolorapply{0.4545} & \cellcolorapply{0.2657} & \cellcolorapply{0.4237} & \cellcolorapply{0.5407} & \cellcolorapply{0.5032} & \cellcolorapply{0.8736} & \cellcolorapply{0.4000} & \cellcolorapply{0.6425} & \cellcolorapply{0.6461} & \cellcolorapply{0.6977} & \cellcolorapply{0.7166} & \cellcolorapply{0.4200} & \cellcolorapply{0.3763} & \cellcolorapply{0.5014} & \cellcolorapply{0.4423} \\

Qwen2.5-VL-7B   & \cellcolorapply{\avgH} & \cellcolorapply{0.6862} & \cellcolorapply{0.3112} & \cellcolorapply{0.6772} & \cellcolorapply{0.7031} & \cellcolorapply{0.3000} & \cellcolorapply{0.2771} & \cellcolorapply{0.5000} & \cellcolorapply{0.5116} & \cellcolorapply{0.5194} & \cellcolorapply{0.8773} & \cellcolorapply{0.2971} & \cellcolorapply{0.5121} & \cellcolorapply{0.5391} & \cellcolorapply{0.5781} & \cellcolorapply{0.6073} & \cellcolorapply{0.3543} & \cellcolorapply{0.2712} & \cellcolorapply{0.4901} & \cellcolorapply{0.4183} \\

Qwen2.5-VL-32B  & \cellcolorapply{\avgD} & \cellcolorapply{0.6695} & \cellcolorapply{0.2963} & \cellcolorapply{0.6888} & \cellcolorapply{0.7656} & \cellcolorapply{0.4879} & \cellcolorapply{0.1914} & \cellcolorapply{0.3644} & \cellcolorapply{0.4767} & \cellcolorapply{0.5290} & \cellcolorapply{0.8953} & \cellcolorapply{0.4029} & \cellcolorapply{0.6425} & \cellcolorapply{0.6667} & \cellcolorapply{0.6113} & \cellcolorapply{0.5911} & \cellcolorapply{0.3943} & \cellcolorapply{0.2373} & \cellcolorapply{0.5156} & \cellcolorapply{0.4567} \\

Qwen2.5-VL-72B & \cellcolorapply{\avgB} & \cellcolorapply{0.7029} & \cellcolorapply{0.3478} & \cellcolorapply{0.7176} & \cellcolorapply{0.7562} & \cellcolorapply{0.3545} & \cellcolorapply{0.2429} & \cellcolorapply{0.3814} & \cellcolorapply{0.5058} & \cellcolorapply{0.5774} & \cellcolorapply{0.2527} & \cellcolorapply{0.2514} & \cellcolorapply{0.6425} & \cellcolorapply{0.7160} & \cellcolorapply{0.6645} & \cellcolorapply{0.7287} & \cellcolorapply{0.5612} & \cellcolorapply{0.3525} & \cellcolorapply{0.5071} & \cellcolorapply{0.4760} \\

InternVL3.5-8B & \cellcolorapply{\avgF} & \cellcolorapply{0.5816} & \cellcolorapply{0.2706} & \cellcolorapply{0.7262} & \cellcolorapply{0.6812} & \cellcolorapply{0.3636} & \cellcolorapply{0.1771} & \cellcolorapply{0.3475} & \cellcolorapply{0.4884} & \cellcolorapply{0.3677} & \cellcolorapply{0.8809} & \cellcolorapply{0.3400} & \cellcolorapply{0.4928} & \cellcolorapply{0.5473} & \cellcolorapply{0.5626} & \cellcolorapply{0.6073} & \cellcolorapply{0.3457} & \cellcolorapply{0.4068} & \cellcolorapply{0.3966} & \cellcolorapply{0.3702} \\

InternVL3.5-38B & \cellcolorapply{\avgF} & \cellcolorapply{0.4686} & \cellcolorapply{0.2233} & \cellcolorapply{0.5504} & \cellcolorapply{0.6656} & \cellcolorapply{0.4909} & \cellcolorapply{0.1829} & \cellcolorapply{0.2797} & \cellcolorapply{0.2965} & \cellcolorapply{0.4762} & \cellcolorapply{0.6318} & \cellcolorapply{0.2457} & \cellcolorapply{0.5217} & \cellcolorapply{0.6708} & \cellcolorapply{0.5947} & \cellcolorapply{0.6356} & \cellcolorapply{0.3514} & \cellcolorapply{0.3254} & \cellcolorapply{0.2408} & \cellcolorapply{0.4038} \\

InternVL3-14B & \cellcolorapply{\avgE} & \cellcolorapply{0.6653} & \cellcolorapply{0.1840} & \cellcolorapply{0.7205} & \cellcolorapply{0.7375} & \cellcolorapply{0.3242} & \cellcolorapply{0.1629} & \cellcolorapply{0.4153} & \cellcolorapply{0.5407} & \cellcolorapply{0.3387} & \cellcolorapply{0.8628} & \cellcolorapply{0.4200} & \cellcolorapply{0.5652} & \cellcolorapply{0.5844} & \cellcolorapply{0.4784} & \cellcolorapply{0.5425} & \cellcolorapply{0.3571} & \cellcolorapply{0.2949} & \cellcolorapply{0.3626} & \cellcolorapply{0.3462} \\

InternVL3-78B & \cellcolorapply{\avgC} & \cellcolorapply{0.7280} & \cellcolorapply{0.5223} & \cellcolorapply{0.6686} & \cellcolorapply{0.5844} & \cellcolorapply{0.4545} & \cellcolorapply{0.1600} & \cellcolorapply{0.5000} & \cellcolorapply{0.4593} & \cellcolorapply{0.4065} & \cellcolorapply{0.8809} & \cellcolorapply{0.4886} & \cellcolorapply{0.5942} & \cellcolorapply{0.7325} & \cellcolorapply{0.6977} & \cellcolorapply{0.6964} & \cellcolorapply{0.4086} & \cellcolorapply{0.3864} & \cellcolorapply{0.4618} & \cellcolorapply{0.3462} \\

LLaVA-OneVision-7B & \cellcolorapply{\avgH} & \cellcolorapply{0.6276} & \cellcolorapply{0.1813} & \cellcolorapply{0.6974} & \cellcolorapply{0.6594} & \cellcolorapply{0.2515} & \cellcolorapply{0.2429} & \cellcolorapply{0.4068} & \cellcolorapply{0.4884} & \cellcolorapply{0.4226} & \cellcolorapply{0.5560} & \cellcolorapply{0.2771} & \cellcolorapply{0.3188} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.0000} & \cellcolorapply{0.2886} & \cellcolorapply{0.2746} & \cellcolorapply{0.4136} & \cellcolorapply{0.4663} \\

MiniCPM-V-4.5-8B & \cellcolorapply{\avgG} & \cellcolorapply{0.6318} & \cellcolorapply{0.3627} & \cellcolorapply{0.7205} & \cellcolorapply{0.7250} & \cellcolorapply{0.3879} & \cellcolorapply{0.2714} & \cellcolorapply{0.3814} & \cellcolorapply{0.4477} & \cellcolorapply{0.4806} & \cellcolorapply{0.5668} & \cellcolorapply{0.3457} & \cellcolorapply{0.3816} & \cellcolorapply{0.6049} & \cellcolorapply{0.6080} & \cellcolorapply{0.5628} & \cellcolorapply{0.3314} & \cellcolorapply{0.3932} & \cellcolorapply{0.4278} & \cellcolorapply{0.4327} \\

MiMo-VL-7B-RL & \cellcolorapply{\avgH} & \cellcolorapply{0.6736} & \cellcolorapply{0.2422} & \cellcolorapply{0.6888} & \cellcolorapply{0.7062} & \cellcolorapply{0.1697} & \cellcolorapply{0.3143} & \cellcolorapply{0.4322} & \cellcolorapply{0.3256} & \cellcolorapply{0.4806} & \cellcolorapply{0.8448} & \cellcolorapply{0.2914} & \cellcolorapply{0.5411} & \cellcolorapply{0.4074} & \cellcolorapply{0.3920} & \cellcolorapply{0.3684} & \cellcolorapply{0.4000} & \cellcolorapply{0.2373} & \cellcolorapply{0.4844} & \cellcolorapply{0.4231} \\

\bottomrule
\end{tabular}
\end{adjustbox}
\endgroup % ========== 局部作用域结束 ==========
\caption{Zero-shot accuracy on \textbf{\OURS}. Color encodes accuracy (yellow$\to$red; higher is redder). The full names of the tasks (from left to right) are: Scene Classification, Object Classification, Environment State Classification, Visual Localization, Urban OCR, Class-agnostic Counting, Referring Expression Counting, Target Backtracking, Cross-Object Reasoning, Intent Analysis and Prediction, Scene Function and Attribute Recognition, Scene Anomaly Analysis, Scene Analysis and Prediction, Event Tracing, Event Understanding, Event Prediction, Multi-Image Sorting, Swarm Collaborative Planning, Semantic-Guided Planning, and Situation Responsive Collaborative Planning.}
\label{tab:zero_shot_all}
\end{table*}

